VMID: A Multimodal Fusion LLM Framework for Detecting and Identifying Misinformation of Short Videos

Short video platforms have become important channels for news dissemination, offering a highly engaging and immediate way for users to access current events and share information. However, these platforms have also emerged as significant conduits for the rapid spread of misinformation, as fake news and rumors can leverage the visual appeal and wide reach of short videos to circulate extensively among audiences. Existing fake news detection methods mainly rely on single-modal information, such as text or images, or apply only basic fusion techniques, limiting their ability to handle the complex, multi-layered information inherent in short videos. To address these limitations, this paper presents a novel fake news detection method based on multimodal information, designed to identify misinformation through a multi-level analysis of video content. This approach effectively utilizes different modal representations to generate a unified textual description, which is then fed into a large language model for comprehensive evaluation. The proposed framework successfully integrates multimodal features within videos, significantly enhancing the accuracy and reliability of fake news detection. Experimental results demonstrate that the proposed approach outperforms existing models in terms of accuracy, robustness, and utilization of multimodal information, achieving an accuracy of 90.93%, which is significantly higher than the best baseline model (SV-FEND) at 81.05%. Furthermore, case studies provide additional evidence of the effectiveness of the approach in accurately distinguishing between fake news, debunking content, and real incidents, highlighting its reliability and robustness in real-world applications.

==> discuss.tex <==
% Although it is shown in the evaluation part that our proposed approach and implementation can have a sound effect against dangerous smart home apps, however, as aforementioned, our approach cannot defend against open-port based attacks due to the reasons illustrated in Section~\ref{sec:background}. Fortunately, there are multiple alternatives that may have the potential to mitigate these attacks. 
% \begin{itemize}
% \item \textbf{Inhibiting Dictionary Attacks.} Dictionary attacks is the first step that Mirai took to compromise IoT devices~\cite{mirai}. Therefore, inhibiting dictionary attacks may effectively hinder Mirai and similar botnets exploiting weak credentials. Currently, multiple solutions have been proposed to inhibit the dictionary attacks from different aspects~\cite{bontrager2018}\cite{2016wuhiera}. Yet, these solutions are mainly designed for general-purpose computing systems. Whether or not they can be migrated to the embedded systems needs to be further scrutinized.

% \item \textbf{Code-Level Vulnerability Discovery.} Sophisticated botnets (e.g., IoTReaper) exploits a number of zero-day vulnerabilities to compromise IoT devices~\cite{greenberg2017reaper}. Therefore, code-level bug searching techniques may serve as ideal solutions to mitigate the zero-day based open-port attacks~\cite{shoshitaishvili2015firmalice}\cite{muench2018you}\cite{Zheng2017usenix}.

% \item \textbf{Hardware-Assisted Approaches.} Some zero-day vulnerabilities may be too complicated to be uncovered using merely the static code-level analysis. In this case, leveraging hardware as an assistant to isolate sensitive information/codes from the insensitive ones can constrain the damages brought by the zero-day vulnerabilities~\cite{Frassetto2018imix}\cite{weiser2019timber}. 
% \end{itemize}
